String graphs with precise number of intersections

A string graph is an intersection graph of curves in the plane. A $k$-string graph is a graph with a string representation in which every pair of curves intersects in at most $k$ points. We introduce the class of $(=k)$-string graphs as a further restriction of $k$-string graphs by requiring that every two curves intersect in either zero or precisely $k$ points. We study the hierarchy of these graphs, showing that for any $k\geq 1$, $(=k)$-string graphs are a subclass of $(=k+2)$-string graphs as well as of $(=4k)$-string graphs; however, there are no other inclusions between the classes of $(=k)$-string and $(=\ell)$-string graphs apart from those that are implied by the above rules. In particular, the classes of $(=k)$-string graphs and $(=k+1)$-string graphs are incomparable by inclusion for any $k$, and the class of $(=2)$-string graphs is not contained in the class of $(=2\ell+1)$-string graphs for any $\ell$.

==> img/Lgraphcompletekpartiteblowup.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \draw
    (64, 736)
     -- (64, 704)
     -- (160, 704);
  \draw
    (96, 736)
     -- (96, 672)
     -- (160, 672);
  \draw
    (128, 736)
     -- (128, 640)
     -- (160, 640);
  \draw
    (200, 736)
     -- (200, 712)
     -- (288, 712);
  \draw
    (192, 736)
     -- (192, 704)
     -- (288, 704);
  \draw
    (208, 736)
     -- (208, 720)
     -- (288, 720);
  \draw
    (224, 736)
     -- (224, 672)
     -- (288, 672);
  \draw
    (232, 736)
     -- (232, 680)
     -- (288, 680);
  \draw
    (256, 736)
     -- (256, 640)
     -- (288, 640);
  \draw
    (288, 648)
     -- (264, 648)
     -- (264, 736);
  \draw
    (248, 736)
     -- (248, 632)
     -- (288, 632);
  \draw
    (272, 736)
     -- (272, 656)
     -- (288, 656);
  \draw[->]
    (168, 688)
     -- (184, 688);
\end{tikzpicture}


==> img/intervalpurification.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \draw
    (96, 704)
     -- (256, 704);
  \draw
    (128, 720)
     -- (128, 608)
     -- (128, 608);
  \draw
    (208, 720)
     -- (208, 608);
  \draw
    (112, 672)
     -- (240, 672);
  \draw
    (212, 676)
     -- (212, 620);
  \draw
    (200, 664)
     -- (256, 664);
  \draw
    (320, 704)
     -- (480, 704);
  \draw
    (352, 720)
     -- (352, 608)
     -- (352, 608);
  \draw
    (432, 720)
     -- (432, 608);
  \draw
    (336, 672)
     -- (464, 672);
  \draw
    (424, 640)
     -- (480, 640);
  \draw
    (448, 676)
     -- (448, 620);
  \draw
    (240, 668)
     -- (112, 668);
  \draw
    (464, 656)
     -- (336, 656);
  \draw[->]
    (272, 664)
     -- (304, 664);
  \draw[ipe dash dotted, {<[ipe arrow tiny]}-{>[ipe arrow tiny]}]
    (440, 672)
     -- (440, 656);
  \node[ipe node, anchor=center]
     at (436, 664) {$\varepsilon$};
  \draw[ipe dash dotted, {<[ipe arrow tiny]}-{>[ipe arrow tiny]}]
    (440, 656)
     -- (440, 640);
  \node[ipe node, anchor=center]
     at (436, 648) {$\varepsilon$};
  \draw[shift={(448, 632)}, rotate=-90, ipe dash dotted, {<[ipe arrow tiny]}-{>[ipe arrow tiny]}]
    (0, 0)
     -- (0, -16);
  \node[ipe node, anchor=center]
     at (440, 628) {$\varepsilon$};
\end{tikzpicture}


==> img/noodleexample1.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet,scale=0.7, every node/.style={scale=0.7}]
  \draw
    (276, 696)
     -- (300, 696);
  \draw
    (280, 700)
     -- (280, 688);
  \draw
    (296, 700)
     -- (296, 688);
  \draw
    (288, 708)
     -- (288, 680);
  \draw
    (284, 684)
     -- (296, 684);
  \draw
    (292, 692)
     -- (320, 692);
  \draw
    (312, 696)
     -- (336, 696);
  \draw
    (316, 700)
     -- (316, 688);
  \draw
    (324, 708)
     -- (324, 680);
  \draw
    (320, 684)
     -- (332, 684);
  \draw
    (240, 696)
     -- (264, 696);
  \draw
    (260, 700)
     -- (260, 688);
  \draw
    (252, 708)
     -- (252, 680);
  \draw
    (248, 684)
     -- (260, 684);
  \draw
    (256, 692)
     -- (284, 692);
  \draw
    (256, 688)
     -- (256, 664);
  \draw
    (292, 688)
     -- (292, 664);
  \draw
    (328, 688)
     -- (328, 664);
  \draw
    (276, 660)
     -- (300, 660);
  \draw
    (280, 664)
     -- (280, 652);
  \draw
    (296, 664)
     -- (296, 652);
  \draw
    (284, 668)
     -- (296, 668);
  \draw
    (288, 672)
     -- (288, 644);
  \draw
    (284, 648)
     -- (296, 648);
  \draw
    (292, 656)
     -- (320, 656);
  \draw
    (312, 660)
     -- (336, 660);
  \draw
    (316, 664)
     -- (316, 652);
  \draw
    (320, 668)
     -- (332, 668);
  \draw
    (324, 672)
     -- (324, 644);
  \draw
    (320, 648)
     -- (332, 648);
  \draw
    (240, 660)
     -- (264, 660);
  \draw
    (260, 664)
     -- (260, 652);
  \draw
    (248, 668)
     -- (260, 668);
  \draw
    (252, 672)
     -- (252, 644);
  \draw
    (248, 648)
     -- (260, 648);
  \draw
    (256, 656)
     -- (284, 656);
  \draw
    (256, 652)
     -- (256, 628);
  \draw
    (292, 652)
     -- (292, 628);
  \draw
    (328, 652)
     -- (328, 628);
  \draw
    (276, 624)
     -- (300, 624);
  \draw
    (280, 628)
     -- (280, 616);
  \draw
    (296, 628)
     -- (296, 616);
  \draw
    (284, 632)
     -- (296, 632);
  \draw
    (288, 636)
     -- (288, 608);
  \draw
    (292, 620)
     -- (320, 620);
  \draw
    (312, 624)
     -- (336, 624);
  \draw
    (316, 628)
     -- (316, 616);
  \draw
    (320, 632)
     -- (332, 632);
  \draw
    (324, 636)
     -- (324, 608);
  \draw
    (240, 624)
     -- (264, 624);
  \draw
    (260, 628)
     -- (260, 616);
  \draw
    (248, 632)
     -- (260, 632);
  \draw
    (252, 636)
     -- (252, 608);
  \draw
    (256, 620)
     -- (284, 620);
  \draw[->]
    (204, 656)
     -- (228, 656);
  \draw
    (128, 688) rectangle (192, 624);
  \draw
    (160, 688)
     -- (160, 624);
  \draw
    (128, 656)
     -- (192, 656);
  \pic[ipe mark large]
     at (128, 688) {ipe disk};
  \pic[ipe mark large]
     at (160, 688) {ipe disk};
  \pic[ipe mark large]
     at (192, 688) {ipe disk};
  \pic[ipe mark large]
     at (192, 656) {ipe disk};
  \pic[ipe mark large]
     at (192, 624) {ipe disk};
  \pic[ipe mark large]
     at (160, 624) {ipe disk};
  \pic[ipe mark large]
     at (160, 656) {ipe disk};
  \pic[ipe mark large]
     at (128, 656) {ipe disk};
  \pic[ipe mark large]
     at (128, 624) {ipe disk};
\end{tikzpicture}


==> img/noodleextension1.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet,scale=0.7, every node/.style={scale=0.7}]
  \draw
    (80, 608)
     -- (144, 608)
     -- (144, 608);
  \draw
    (128, 592)
     -- (128, 640);
  \draw
    (112, 624)
     -- (240, 624);
  \draw
    (224, 640)
     -- (224, 592);
  \draw
    (208, 608)
     -- (272, 608);
  \draw
    (256, 560)
     -- (256, 672);
  \draw
    (272, 656)
     -- (224, 656);
  \draw
    (240, 640)
     -- (240, 768);
  \draw
    (224, 752)
     -- (272, 752);
  \draw
    (256, 736)
     -- (256, 816);
  \draw
    (96, 560)
     -- (96, 672);
  \draw
    (112, 656)
     -- (64, 656);
  \draw
    (80, 640)
     -- (80, 768);
  \draw
    (64, 752)
     -- (112, 752);
  \draw
    (96, 736)
     -- (96, 816);
  \draw
    (80, 784)
     -- (144, 784)
     -- (144, 784);
  \draw
    (128, 768)
     -- (128, 816);
  \draw
    (112, 800)
     -- (240, 800);
  \draw
    (224, 816)
     -- (224, 768);
  \draw
    (208, 784)
     -- (272, 784);
  \draw[ipe pen fat]
    (96, 720)
     -- (48, 720);
  \draw[ipe pen fat]
    (48, 688)
     -- (176, 688)
     -- (176, 576);
  \draw
    (368, 608)
     -- (432, 608)
     -- (432, 608);
  \draw
    (416, 592)
     -- (416, 640);
  \draw
    (400, 624)
     -- (528, 624);
  \draw
    (512, 640)
     -- (512, 592);
  \draw
    (496, 608)
     -- (560, 608);
  \draw
    (544, 560)
     -- (544, 672);
  \draw
    (560, 656)
     -- (512, 656);
  \draw
    (528, 640)
     -- (528, 768);
  \draw
    (512, 752)
     -- (560, 752);
  \draw
    (544, 736)
     -- (544, 816);
  \draw
    (384, 560)
     -- (384, 672);
  \draw
    (400, 656)
     -- (352, 656);
  \draw
    (368, 640)
     -- (368, 768);
  \draw
    (352, 752)
     -- (400, 752);
  \draw
    (384, 736)
     -- (384, 816);
  \draw
    (368, 784)
     -- (432, 784)
     -- (432, 784);
  \draw
    (416, 768)
     -- (416, 816);
  \draw
    (400, 800)
     -- (528, 800);
  \draw
    (512, 816)
     -- (512, 768);
  \draw
    (496, 784)
     -- (560, 784);
  \draw[ipe pen fat]
    (384, 720)
     -- (336, 720);
  \draw[ipe pen fat]
    (336, 688)
     -- (464, 688)
     -- (464, 576);
  \draw
    (416, 640)
     -- (420, 640)
     -- (420, 616)
     -- (424, 616)
     -- (424, 640)
     -- (428, 640)
     -- (428, 616);
  \draw
    (416, 592)
     -- (412, 592)
     -- (412, 616)
     -- (408, 616)
     -- (408, 592)
     -- (404, 592)
     -- (404, 616);
  \draw
    (352, 656)
     -- (352, 660)
     -- (376, 660)
     -- (376, 664)
     -- (352, 664)
     -- (352, 668)
     -- (376, 668);
  \draw
    (400, 656)
     -- (400, 652)
     -- (376, 652)
     -- (376, 648)
     -- (400, 648)
     -- (400, 644)
     -- (376, 644);
  \draw
    (512, 592)
     -- (508, 592)
     -- (508, 616)
     -- (504, 616)
     -- (504, 592)
     -- (500, 592)
     -- (500, 616);
  \draw
    (512, 640)
     -- (516, 640)
     -- (516, 616)
     -- (520, 616)
     -- (520, 640)
     -- (524, 640)
     -- (524, 616);
  \draw
    (512, 656)
     -- (512, 652)
     -- (536, 652)
     -- (536, 648)
     -- (512, 648)
     -- (512, 644)
     -- (536, 644);
  \draw
    (560, 656)
     -- (560, 660)
     -- (536, 660)
     -- (536, 664)
     -- (556, 664)
     -- (560, 664)
     -- (560, 668)
     -- (536, 668);
  \draw
    (560, 752)
     -- (560, 748)
     -- (536, 748)
     -- (536, 744)
     -- (560, 744)
     -- (560, 740)
     -- (536, 740);
  \draw
    (512, 752)
     -- (512, 756)
     -- (536, 756)
     -- (536, 760)
     -- (512, 760)
     -- (512, 764)
     -- (536, 764);
  \draw
    (512, 816)
     -- (516, 816)
     -- (516, 792)
     -- (520, 792)
     -- (520, 816)
     -- (524, 816)
     -- (524, 792);
  \draw
    (416, 816)
     -- (412, 816)
     -- (412, 792)
     -- (408, 792)
     -- (408, 816)
     -- (404, 816)
     -- (404, 792);
  \draw
    (416, 768)
     -- (420, 768)
     -- (420, 792)
     -- (424, 792)
     -- (424, 768)
     -- (428, 768)
     -- (428, 792);
  \draw
    (352, 752)
     -- (352, 756)
     -- (376, 756)
     -- (376, 760)
     -- (352, 760)
     -- (352, 764)
     -- (376, 764);
  \draw
    (400, 752)
     -- (400, 748)
     -- (376, 748)
     -- (376, 744)
     -- (400, 744)
     -- (400, 740)
     -- (376, 740);
  \draw
    (512, 768)
     -- (508, 768)
     -- (508, 792)
     -- (504, 792)
     -- (504, 768)
     -- (500, 768)
     -- (500, 792);
  \draw
    (368, 784)
     -- (368, 788)
     -- (392, 788)
     -- (392, 792)
     -- (368, 792)
     -- (368, 796)
     -- (392, 796);
  \draw
    (560, 784)
     -- (560, 788)
     -- (536, 788)
     -- (536, 792)
     -- (560, 792)
     -- (560, 796)
     -- (536, 796);
  \draw
    (560, 608)
     -- (560, 604)
     -- (536, 604)
     -- (536, 600)
     -- (560, 600)
     -- (560, 596)
     -- (536, 596);
  \draw[->]
    (272, 704)
     -- (336, 704);
  \draw
    (432, 608)
     -- (432, 588)
     -- (372, 588)
     -- (372, 584)
     -- (396, 584)
     -- (396, 580)
     -- (372, 580);
\end{tikzpicture}


==> img/noodleextension2.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet,scale=0.7, every node/.style={scale=0.7}]
  \draw
    (96, 592)
     -- (160, 592)
     -- (160, 592);
  \draw
    (144, 576)
     -- (144, 624);
  \draw
    (128, 608)
     -- (256, 608);
  \draw
    (240, 624)
     -- (240, 576);
  \draw
    (224, 592)
     -- (288, 592);
  \draw
    (272, 544)
     -- (272, 656);
  \draw
    (288, 640)
     -- (240, 640);
  \draw
    (256, 624)
     -- (256, 752);
  \draw
    (240, 736)
     -- (288, 736);
  \draw
    (272, 720)
     -- (272, 800);
  \draw
    (112, 544)
     -- (112, 656);
  \draw
    (128, 640)
     -- (80, 640);
  \draw
    (96, 624)
     -- (96, 752);
  \draw
    (80, 736)
     -- (128, 736);
  \draw
    (112, 720)
     -- (112, 800);
  \draw
    (96, 768)
     -- (160, 768)
     -- (160, 768);
  \draw
    (144, 752)
     -- (144, 800);
  \draw
    (128, 784)
     -- (256, 784);
  \draw
    (240, 800)
     -- (240, 752);
  \draw
    (224, 768)
     -- (288, 768);
  \draw[ipe pen fat]
    (112, 704)
     -- (64, 704);
  \draw[ipe pen fat]
    (64, 672)
     -- (192, 672)
     -- (192, 560);
  \draw
    (384, 592)
     -- (448, 592)
     -- (448, 592);
  \draw
    (432, 576)
     -- (432, 624);
  \draw
    (416, 608)
     -- (544, 608);
  \draw
    (528, 624)
     -- (528, 576);
  \draw
    (512, 592)
     -- (576, 592);
  \draw
    (560, 544)
     -- (560, 656);
  \draw
    (576, 640)
     -- (528, 640);
  \draw
    (544, 624)
     -- (544, 752);
  \draw
    (528, 736)
     -- (576, 736);
  \draw
    (560, 720)
     -- (560, 800);
  \draw
    (400, 544)
     -- (400, 656);
  \draw
    (416, 640)
     -- (368, 640);
  \draw
    (384, 624)
     -- (384, 752);
  \draw
    (368, 736)
     -- (416, 736);
  \draw
    (400, 720)
     -- (400, 800);
  \draw
    (384, 768)
     -- (448, 768)
     -- (448, 768);
  \draw
    (432, 752)
     -- (432, 800);
  \draw
    (416, 784)
     -- (544, 784);
  \draw
    (528, 800)
     -- (528, 752);
  \draw
    (512, 768)
     -- (576, 768);
  \draw[ipe pen fat]
    (400, 704)
     -- (352, 704);
  \draw[ipe pen fat]
    (352, 672)
     -- (480, 672)
     -- (480, 560);
  \draw
    (432, 624)
     -- (436, 624)
     -- (436, 600)
     -- (440, 600)
     -- (440, 624)
     -- (444, 624)
     -- (444, 600);
  \draw
    (432, 576)
     -- (428, 576)
     -- (428, 600)
     -- (424, 600)
     -- (424, 576)
     -- (420, 576)
     -- (420, 600);
  \draw
    (368, 640)
     -- (368, 644)
     -- (392, 644)
     -- (392, 648)
     -- (368, 648)
     -- (368, 652)
     -- (392, 652);
  \draw
    (416, 640)
     -- (416, 636)
     -- (392, 636)
     -- (392, 632)
     -- (416, 632)
     -- (416, 628)
     -- (392, 628);
  \draw
    (528, 576)
     -- (524, 576)
     -- (524, 600)
     -- (520, 600)
     -- (520, 576)
     -- (516, 576)
     -- (516, 600);
  \draw
    (528, 624)
     -- (532, 624)
     -- (532, 600)
     -- (536, 600)
     -- (536, 624)
     -- (540, 624)
     -- (540, 600);
  \draw
    (528, 640)
     -- (528, 636)
     -- (552, 636)
     -- (552, 632)
     -- (528, 632)
     -- (528, 628)
     -- (552, 628);
  \draw
    (576, 640)
     -- (576, 644)
     -- (552, 644)
     -- (552, 648)
     -- (572, 648)
     -- (576, 648)
     -- (576, 652)
     -- (552, 652);
  \draw
    (576, 736)
     -- (576, 732)
     -- (552, 732)
     -- (552, 728)
     -- (576, 728)
     -- (576, 724)
     -- (552, 724);
  \draw
    (528, 736)
     -- (528, 740)
     -- (552, 740)
     -- (552, 744)
     -- (528, 744)
     -- (528, 748)
     -- (552, 748);
  \draw
    (528, 800)
     -- (532, 800)
     -- (532, 776)
     -- (536, 776)
     -- (536, 800)
     -- (540, 800)
     -- (540, 776);
  \draw
    (432, 800)
     -- (428, 800)
     -- (428, 776)
     -- (424, 776)
     -- (424, 800)
     -- (420, 800)
     -- (420, 776);
  \draw
    (432, 752)
     -- (436, 752)
     -- (436, 776)
     -- (440, 776)
     -- (440, 752)
     -- (444, 752)
     -- (444, 776);
  \draw
    (368, 736)
     -- (368, 740)
     -- (392, 740)
     -- (392, 744)
     -- (368, 744)
     -- (368, 748)
     -- (392, 748);
  \draw
    (416, 736)
     -- (416, 732)
     -- (392, 732)
     -- (392, 728)
     -- (416, 728)
     -- (416, 724)
     -- (392, 724);
  \draw
    (416, 608)
     -- (416, 624)
     -- (424, 624)
     -- (424, 636)
     -- (492, 636)
     -- (492, 632)
     -- (468, 632)
     -- (468, 628)
     -- (492, 628);
  \draw
    (384, 624)
     -- (356, 624)
     -- (356, 680)
     -- (364, 680)
     -- (364, 660);
  \draw
    (528, 752)
     -- (524, 752)
     -- (524, 776)
     -- (520, 776)
     -- (520, 752)
     -- (516, 752)
     -- (516, 776);
  \draw
    (384, 768)
     -- (384, 772)
     -- (408, 772)
     -- (408, 776)
     -- (384, 776)
     -- (384, 780)
     -- (408, 780);
  \draw
    (576, 768)
     -- (576, 772)
     -- (552, 772)
     -- (552, 776)
     -- (576, 776)
     -- (576, 780)
     -- (552, 780);
  \draw
    (576, 592)
     -- (576, 588)
     -- (552, 588)
     -- (552, 584)
     -- (576, 584)
     -- (576, 580)
     -- (552, 580);
  \draw[->]
    (288, 688)
     -- (352, 688);
  \draw
    (448, 592)
     -- (448, 572)
     -- (388, 572)
     -- (388, 568)
     -- (412, 568)
     -- (412, 564)
     -- (388, 564);
\end{tikzpicture}


==> tikzlibraryipe.code.tex <==

% Copyright (C) 2016  Joseph Rabinoff

% ipe2tikz is free software; you can redistribute it and/or modify it under
% the terms of the GNU General Public License as published by the Free
% Software Foundation; either version 3 of the License, or (at your option)
% any later version.

% ipe2tikz is distributed in the hope that it will be useful, but WITHOUT ANY
% WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the GNU General Public License for more
% details.

% You should have received a copy of the GNU General Public License along with
% ipe2tikz; if not, you can find it at "http://www.gnu.org/copyleft/gpl.html",
% or write to the Free Software Foundation, Inc., 675 Mass Ave, Cambridge, MA
% 02139, USA.


% ipe compatibility TikZ styles

\usetikzlibrary{arrows.meta}

\makeatletter

% These should behave almost exactly like ipe arrows.  They disable correcting
% for the miter length and line width.  This is important for visual consistency
% with ipe, since ipe arrows get much larger when the line width is increased.
% They also use the line join and cap styles from the main path.  These are very
% simple arrows: there is no harpoon version, and the convex hull computation is
% sloppy.

\pgfdeclarearrow{
  name = ipe _linear,
  defaults = {
    length = +1bp,
    width  = +.666bp,
    line width = +0pt 1,
  },
  setup code = {
    % Control points
    \pgfarrowssetbackend{0pt}
    \pgfarrowssetvisualbackend{
      \pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \pgfarrowssetlineend{\pgfarrowlength}
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % Convex hull
    \pgfarrowshullpoint{\pgfarrowlength}{0pt}
    \pgfarrowsupperhullpoint{0pt}{.5\pgfarrowwidth}
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth}}
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
  },
}


\pgfdeclarearrow{
  name = ipe _pointed,
  defaults = {
    length = +1bp,
    width  = +.666bp,
    inset  = +.2bp,
    line width = +0pt 1,
  },
  setup code = {
    % Control points
    \pgfarrowssetbackend{0pt}
    \pgfarrowssetvisualbackend{\pgfarrowinset}
    \pgfarrowssetlineend{\pgfarrowinset}
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % Convex hull
    \pgfarrowshullpoint{\pgfarrowlength}{0pt}
    \pgfarrowsupperhullpoint{0pt}{.5\pgfarrowwidth}
    \pgfarrowshullpoint{\pgfarrowinset}{0pt}
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowinset
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowinset}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth}}
    \pgfpathclose
    \ifpgfarrowopen
      \pgfusepathqstroke
    \else
      \ifdim\pgfarrowlinewidth>0pt\pgfusepathqfillstroke\else\pgfusepathqfill\fi
    \fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \the\pgfarrowinset,%
    \ifpgfarrowopen o\fi%
  },
}


% For correcting minipage width in stretched nodes
\newdimen\ipeminipagewidth
\def\ipestretchwidth#1{%
  \pgfmathsetlength{\ipeminipagewidth}{#1/\ipenodestretch}}

\tikzstyle{ipe import} = [
  % General ipe defaults
  x=1bp, y=1bp,
%
  % Nodes
  ipe node stretch/.store in=\ipenodestretch,
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe node/.style={
    anchor=base west, inner sep=0, outer sep=0, scale=\ipenodestretch
  },
%
  % Use a special key for the mark scale, so that the default can be overriden.
  % (This doesn't happen with the scale= key; those accumulate.)
  ipe mark scale/.store in=\ipemarkscale,
%
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
%
  ipe mark normal, % Set default
%
  ipe circle/.pic={
    \draw[line width=0.2*\ipemarkscale]
      (0,0) circle[radius=0.5*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe disk/.pic={
    \fill (0,0) circle[radius=0.6*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe fdisk/.pic={
    \filldraw[line width=0.2*\ipemarkscale]
      (0,0) circle[radius=0.5*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe box/.pic={
    \draw[line width=0.2*\ipemarkscale, line join=miter]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) rectangle
      ( .5*\ipemarkscale, .5*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe square/.pic={
    \fill
      (-.6*\ipemarkscale,-.6*\ipemarkscale) rectangle
      ( .6*\ipemarkscale, .6*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe fsquare/.pic={
    \filldraw[line width=0.2*\ipemarkscale, line join=miter]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) rectangle
      ( .5*\ipemarkscale, .5*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe cross/.pic={
    \draw[line width=0.2*\ipemarkscale, line cap=butt]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) --
      ( .5*\ipemarkscale, .5*\ipemarkscale)
      (-.5*\ipemarkscale, .5*\ipemarkscale) --
      ( .5*\ipemarkscale,-.5*\ipemarkscale);
    \coordinate () at (0,0);
  },
%
  % Arrow sizes (for TikZ arrows)
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=1},
  ipe arrow tiny/.style={scale=.4},
  ipe arrow small/.style={scale=.7},
  ipe arrow large/.style={scale=1.4},
  ipe arrow normal,
  /tikz/.cd,
%
  % Approximations to ipe arrows
  % Put in a style to allow to reset default scale when "ipe arrow normal" is
  % changed.  I think this is the only way, since all the parameters to arrows
  % are expanded when the tip is declared.
  ipe arrows/.style={
    ipe normal/.tip={
      ipe _pointed[length=1bp, width=.666bp, inset=0bp,
                   quick, ipe arrow normal]},
    ipe pointed/.tip={
      ipe _pointed[length=1bp, width=.666bp, inset=0.2bp,
                   quick, ipe arrow normal]},
    ipe linear/.tip={
      ipe _linear[length = 1bp, width=.666bp,
                  ipe arrow normal, quick]},
    ipe fnormal/.tip={ipe normal[fill=white]},
    ipe fpointed/.tip={ipe pointed[fill=white]},
    ipe double/.tip={ipe normal[] ipe normal},
    ipe fdouble/.tip={ipe fnormal[] ipe fnormal},
    % These should maybe use [bend], but that often looks bad unless it's on an
    % actual arc.
    ipe arc/.tip={ipe normal},
    ipe farc/.tip={ipe fnormal},
    ipe ptarc/.tip={ipe pointed},
    ipe fptarc/.tip={ipe fpointed},
  },
  ipe arrows, % Set default sizes
]

% I'm not sure how to do this in a .style, since the #args get confused.
\tikzset{
  rgb color/.code args={#1=#2}{%
    \definecolor{tempcolor-#1}{rgb}{#2}%
    \tikzset{#1=tempcolor-#1}%
  },
}

\makeatother

\endinput

